Multimodal Diffusion Segmentation Model for Object Segmentation from Manipulation Instructions

In this study, we aim to develop a model that comprehends a natural language instruction (e.g., "Go to the living room and get the nearest pillow to the radio art on the wall") and generates a segmentation mask for the target everyday object. The task is challenging because it requires (1) the understanding of the referring expressions for multiple objects in the instruction, (2) the prediction of the target phrase of the sentence among the multiple phrases, and (3) the generation of pixel-wise segmentation masks rather than bounding boxes. Studies have been conducted on languagebased segmentation methods; however, they sometimes mask irrelevant regions for complex sentences. In this paper, we propose the Multimodal Diffusion Segmentation Model (MDSM), which generates a mask in the first stage and refines it in the second stage. We introduce a crossmodal parallel feature extraction mechanism and extend diffusion probabilistic models to handle crossmodal features. To validate our model, we built a new dataset based on the well-known Matterport3D and REVERIE datasets. This dataset consists of instructions with complex referring expressions accompanied by real indoor environmental images that feature various target objects, in addition to pixel-wise segmentation masks. The performance of MDSM surpassed that of the baseline method by a large margin of +10.13 mean IoU.

==> section5.tex <==

\section{Dataset
\label{dataset}
}




==> tab/baseline_comp.tex <==
\begin{table*}[tb]
\centering
%\footnotesize
\caption{
\textbf{Quantitative comparison and ablation studies.}
The methods have been compared on the CoDraw and i-CLEVR datasets according to several metrics:
the average precision~(AP), average recall (AR), F1-score, and relational similarity (RSIM).
For each metric and dataset, the best scores are in bold,
and the second best ones are underlined.
The mean and standard deviation have been calculated on five different seed runs.
% For i-CLEVR, our model boosted the recall by 12.4 point,
% which resulted in the F1 and RSIM are also improved. 
}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{@{}lccccccccc@{}}
\toprule
           & \multicolumn{4}{c}{CoDraw}            & \multicolumn{1}{l}{} & \multicolumn{4}{c}{i-CLEVR}           \\ \cmidrule(lr){2-5} \cmidrule(l){7-10} 
Methods      & AP$\uparrow$ & AR$\uparrow$ & F1$\uparrow$ & RSIM$\uparrow$  &
& AP$\uparrow$ & AR$\uparrow$ & F1$\uparrow$ & RSIM$\uparrow$  \\ \midrule

% fixed (paper result)
GeNeVA-GAN~{\tiny} & 66.64     & 52.66  & 58.83    & 35.41 &                      & 92.39     & 84.72  & 88.39    & 74.02 \\ \midrule

% fixed (single run, actual results)
% Ours (w/o Latte \& TxtCond)   & 75.33  & 74.05  & 71.98  & 47.13  & & 95.19  & 93.92  & 94.45  & 78.28  \\
Ours (w/o Latte \& TxtCond)
& $76.75{\scriptscriptstyle \pm0.94}$    
& $73.99{\scriptscriptstyle \pm0.11}$ 
& $72.81{\scriptscriptstyle \pm0.51}$
& $47.43{\scriptscriptstyle \pm0.28}$  &
& $95.77{\scriptscriptstyle \pm0.59}$
& $94.60{\scriptscriptstyle \pm0.69}$
& $95.08{\scriptscriptstyle \pm0.65}$
& $79.31{\scriptscriptstyle \pm1.23}$ \\

% temporal (single run, expected results (+4, -1, +2, +.5, +3.5, +4, +4, +5))
% \txq{w/o Latte}        & 79.33  & 73.05  & 73.98  & 47.63  & & 98.69  & 97.92  & 98.45  & 83.28  \\
% Ours (w/o Latte)              & 77.82  & 73.54  & 73.03  & 47.96  & & \bf{98.91}  & \bf{98.58}  & \bf{98.72}  & \bf{83.95}  \\
Ours (w/o Latte)
& $79.04{\scriptscriptstyle \pm1.28}$    
& $73.91{\scriptscriptstyle \pm0.53}$ 
& $74.02{\scriptscriptstyle \pm1.03}$
& $48.16{\scriptscriptstyle \pm0.41}$  &
& $\bm{98.35}{\scriptscriptstyle \pm1.27}$
& $\bm{97.68}{\scriptscriptstyle \pm1.61}$
& $\bm{97.96}{\scriptscriptstyle \pm1.47}$
& $\underline{82.78}{\scriptscriptstyle \pm1.94}$ \\

% fixed (single run, actual results)
% Ours (w/o TxtCond)            & \bf{81.48}  & \bf{78.33}  & \bf{77.51}  & 53.41  & & 96.32  & 95.20  & 95.67  & 80.21  \\
Ours (w/o TxtCond)
& $\underline{80.53}{\scriptscriptstyle \pm0.97}$    
& $\bm{78.42}{\scriptscriptstyle \pm0.38}$ 
& $\underline{77.11}{\scriptscriptstyle \pm0.60}$
& $\underline{53.13}{\scriptscriptstyle \pm0.25}$  &
& $96.67{\scriptscriptstyle \pm0.41}$
& $95.52{\scriptscriptstyle \pm0.43}$
& $95.99{\scriptscriptstyle \pm0.42}$
& $81.04{\scriptscriptstyle \pm0.97}$ \\

% temporal (multiple run, expected results (+4, -1, +2, +.5, +3.5, +4, +4, +5))
% \txq{\bf{LatteGAN (Ours)}}
% & ${85.48}{\scriptscriptstyle \pm0.00}$    
% & ${77.33}{\scriptscriptstyle \pm0.00}$ 
% & ${79.51}{\scriptscriptstyle \pm0.00}$
% & ${53.91}{\scriptscriptstyle \pm0.00}$  &
% & ${99.82}{\scriptscriptstyle \pm0.00}$
% & ${99.20}{\scriptscriptstyle \pm0.00}$
% & ${99.67}{\scriptscriptstyle \pm0.00}$
% & ${85.21}{\scriptscriptstyle \pm0.00}$ \\ \bottomrule
\bf{Ours (LatteGAN)}
& $\bm{81.50}{\scriptscriptstyle \pm0.82}$    
& $\underline{78.37}{\scriptscriptstyle \pm0.38}$ 
& $\bm{77.51}{\scriptscriptstyle \pm0.52}$
& $\bm{54.16}{\scriptscriptstyle \pm0.21}$  &
& $\underline{97.72}{\scriptscriptstyle \pm1.44}$
& $\underline{96.93}{\scriptscriptstyle \pm1.64}$
& $\underline{97.26}{\scriptscriptstyle \pm1.56}$
& $\bm{83.21}{\scriptscriptstyle \pm1.70}$ \\ \bottomrule

\end{tabular}
\end{adjustbox}
\label{tab:results}
\end{table*}

==> tab/params.tex <==

\begin{table}[t]
    \centering
    % \vspace{-6mm}
    \caption{\small Parameter settings of the ABEN}
    \vspace{-2mm}
    \small
    \begin{tabular}{|c|l|}
        \hline
         Opt. & Adam ( Learning rate $=1.0 \times 10^{-4},$ \\
         method & $\beta_1=0.7, \beta_2=0.99999$ ) \\ \hline
        Backbone CNN &  ResNet-50 \\ \hline
        % Embedded vector size &  768 \\ \hline
        LSTM & 3 layers, 768-dimensional cell \\ \hline
        $N$ & 10 \\ \hline
        Generation Branch & FC: 768, 768 \\ \hline
        % MLP num. nodes &  [768, 768] \\ \hline
        % input N size &  downscaled to $(224 \times 224 \times 3)$ \\ \hline
        Batch size & 32 \\ \hline
    \end{tabular}
    \label{tab:parameters}
    \vspace{-6mm}
\end{table}


